Octopus: A Multitask Model and Toolkit for Arabic Natural Language Generation

Understanding Arabic text and generating human-like responses is a challenging endeavor. While many researchers have proposed models and solutions for individual problems, there is an acute shortage of a comprehensive Arabic natural language generation toolkit that is capable of handling a wide range of tasks. In this work, we present a novel Arabic text-to-text Transformer model, namely AraT5v2. Our new model is methodically trained on extensive and diverse data, utilizing an extended sequence length of 2,048 tokens. We explore various pretraining strategies including unsupervised, supervised, and joint pertaining, under both single and multitask settings. Our models outperform competitive baselines with large margins. We take our work one step further by developing and publicly releasing Octopus, a Python-based package and command-line toolkit tailored for eight Arabic generation tasks all exploiting a single model. We release the models and the toolkit on our public repository.

==> octopus_tool_usage.tex <==
\section{\octopus: Getting Started} \label{sec:usage}


\subsection{Installation}
% TURJUMAN is implemented in Python and  can be installed using the pip package manager.\footnote{\textit{pip install turjuman}} It is compatible with \textit{Python 3.6} and later versions, \textit{Torch 1.8.1}, and \textit{HuggingFace Transformers 4.5.1 library}.\footnote{Installation instructions and documentation can be found at:~\url{https://github.com/UBC-NLP/turjuman}.}



\octopus~is implemented in Python and can be easily installed using the pip package manager with the following command. It is compatible with Python versions 3.8 and later, Torch version 2.0 and later, and the HuggingFace Transformers library version 4.30 or higher.\footnote{Installation instructions and documentation can be found at:~\url{anonymity_url}.}

% \begin{minted}
% [
% frame=lines,
% framesep=2mm,
% baselinestretch=1.2,
% bgcolor=LightGray,
% fontsize=\footnotesize,
% linenos,
% rulecolor=\color{red}
% ]
% {python}

% \begin{minted}[bgcolor=bg,
%                frame=lines,
%                framesep=2mm]{python}
% pip install octopus
% \end{minted}


\begin{lstlisting}
> pip install octopus 
\end{lstlisting}

\subsection{\octopus~Command Line Examples}


As mentioned earlier, \octopus~offers several command-line tools for multiple generation tasks, each supporting multiple arguments. In the following section, we provide examples demonstrating the usage of these tools with different arguments.\\

\noindent\textbf{Interactive Mode.} In the following example, we use \textit{octopus\_interactive} command line to perform Grammarly checks and then diacritize the input text. Here, we use the default setting which is beam search with a beam size of $5$, a maximum sequence length of $300$, and a number of targets to output at $3$.
\hl{this is initial and will be updated once the later}
\begin{lstlisting}
> octopus_interactive
\end{lstlisting}
\textcolor{blue}{Output------------------------------------------------}
\begin{topbot}
\small
$>$ \texttt{Octopus Interactive CLI} \\
$>$ \texttt{Loading model from UBC-NLP/octopus} \\
$>$ \texttt{\textcolor{red}{Type your task(s) correct-grammar, diacritize}}\\\\
$>$ \texttt{\textcolor{red}{Type your source text or (q) to STOP:}} \\\\
$>$ \texttt{\textbf{She thought a dark moment in her past was forgotten.}} \\
$>$ \texttt{\textcolor{green}{\textbf{target1}}: \<اعتقدت أن لحظة مظلمة في ماضيها قد نسيت.>}\\ 
$>$ \texttt{\textcolor{green}{\textbf{target2}}: \<لقد اعتقدت أن لحظة مظلمة في ماضيها قد نسيت.>}\\ 
$>$ \texttt{\textcolor{green}{\textbf{target3}}: \<كانت تعتقد أن لحظة مظلمة في ماضيها قد نسيت.>}\\\\
$>$ \texttt{\textcolor{red}{Type your source text or (q) to STOP:}} \\
$>$ \texttt{\textbf{Esta é uma lista de estados soberanos}} \\
$>$ \texttt{\textcolor{green}{\textbf{target1}}: \<هذه قائمة الدول ذات السيادة>}\\ 
$>$ \texttt{\textcolor{green}{\textbf{target2}}: \<هذه قائمة بالدول ذات السيادة>}\\ 
$>$ \texttt{\textcolor{green}{\textbf{target3}}: \<قائمة الدول ذات السيادة هذه>}\\ 
\end{topbot}


==> temp_to_remove.tex <==
\section{AraT5\textsubscript{v2}}\label{sec:arat5}




In this section, we introduce a novel iteration of the AraT5, an Arabic-specific sequence-to-sequence  language model proposed by ~\citet{nagoudi-etal-2022-arat5},  we refer to this iteration as AraT5\textsubscript{v2}. AraT5\textsubscript{v2} represents a substantial evolution of the original AraT5 model, marked by notable enhancements. These enhancements include 1) Training on an expanded dataset comprising both labeled and unlabeled data. 2) Larger architecture, incorporating a diverse ensemble of \hl{XX} models, varying in size from \hl{XX} million to \hl{YY} billion parameters. 3) Diverse training strategies that integrate a combination of unsupervised and supervised training techniques.




 % This architectural augmentation contributes to the model's improved performance.
% In this section we describe a a new version of AraT5 proposed by~\newcite{nagoudi-etal-2022-arat5}, namely (AraT5\textsubscript{v2}). AraT5\textsubscript{v2} is trained on larger data (unlabeled and labeled) using unsupervised and supervised training strategies. 
% In this section, we present a novel iteration of AraT5 \citet{nagoudi-etal-2022-arat5} sequence-to-sequence models designed for Arabic, referred to as AraT5\textsubscript{v2}. AraT5\textsubscript{v2}  a is an enhanced version of AraT5~\citet{nagoudi-etal-2022-arat5} trained using: 1) An expanded dataset consisting of both unlabeled and labeled data. 2) Larger architecture with a set of \hl{XX} language models designed for Arabic, varying in size from   \hl{XX}M to \hl{YY}B parameters. 3) Diverse training objectives that integrate a blend of unsupervised and supervised training techniques.


\subsection{Pretraining Data}\label{sub_sec:lm_data}

As we mentioned previously, our pretraining (unlabeled and labeled) dataset is linguistically diverse, covering all categories of Arabic (i.e., CA, DA, and MSA). as we will now describe.

\noindent\textbf{Unlabled Data.}We collect approximately \hl{$XX$} GB of Arabic text, which corresponds to around \hl{$XX$}  billion tokens.  For the MSA and dialect data, we use different sources including  AraNews\textsubscript{v2}\cite{nagoudi2020machine}, El-Khair\cite{elkhair-2016}, Gigaword,\footnote{\href{https://catalog.ldc.upenn.edu/LDC2009T30}{https://catalog.ldc.upenn.edu/LDC2009T30}.} OSIAN~\cite{zeroual2019osian}, Wikipedia Arabic,  Hindawi Books\footnote{\href{https://www.hindawi.org/books/}{https://www.hindawi.org/books}.}, OSCAR\textsubscript{Egyptian}~\cite{suarez2019asynchronous}, and AraC4~\cite{nagoudi2022jasmine}.\footnote{We note that AraC4 contains a diverse Arabic dialect as described in ~\cite{nagoudi2022jasmine}.} To obtain the Classical Arabic (CA) dataset, we utilize the Open Islamicate Texts Initiative (OpenITI) corpus (v1.6)~\cite{nigst2020openiti}. The OpenITI corpus consists of $11$K  Islamic books, primarily collected from sources such as Shamela Liberay,\footnote{\href{https://shamela.ws}{https://shamela.ws}.} Al-Jami Al-Kabir collection (JK),\footnote{\href{http://kitab-project.org/docs/openITI}{http://kitab-project.org/docs/openITI}.} books digitized by the Jordanian publisher Markaz Al-Turāth, and the Shia Library.\footnote{\href{https://shiaonlinelibrary.com}{https://shiaonlinelibrary.com}.}

\noindent\textbf{Labeled Data.}
Recently, \newcite{nagoudi2023dolphin} introduced Dolphin, a natural language generation benchmark for Arabic.  Dolphin covers MSA, Classical Arabic, and various Arabic dialects and it is composed of  $40$ datasets, making it the largest and most diverse Arabic NLG benchmark. Dolphin consists of  $13$ NLP tasks. In our work, we use \textit{8}  out of \textit{$13$} NLG task extracted from the Dolphin benchmark: (1) \textit{text summarisation}, (2) \textit{news title generation}, (3) \textit{question answering}, (4) \textit{question generation}, (5) \textit{transliteration}, (6) \textit{paraphrasing}, (7) \textit{diacritization}, and (8) \textit{grammatical error correction}. Next, we briefly describe each of these tasks.
\section{Training Strategies}\label{sec:traini_Stra}


\subsection{Unsupervised Pretraining.} In this setting, we focus on using only our unlabeled data described in Section~\ref{sub_sec:lm_data} for pre-training our AraT5\textsubscript{v2}. The objective function does not rely on labels but instead imparts the model with transferable knowledge that can be effectively applied to various downstream tasks.  We follow \newcite{raffel2019exploring}
using a masked language modeling ``span-corruption'' objective.  This approach involves replacing consecutive spans of input tokens with a mask token, and the model is trained to reconstruct the masked tokens.

\subsection{Supervised Finetuning.} 

We use the  labeled data (see Section~\ref{sub_sec:lm_data}) to fine-tune the AraT5\textsubscript{v2} models under two settings: (i) single task
and (ii) multi-task. For all experiments, we consistently identify the best checkpoint for each model based on the development set. The performance of each model is then reported on both the development and test data.


\noindent\textbf{Single Task Finetuning.} We individually fine-tune our AraT5\textsubscript{v2}  models on each of the eight NLG tasks of Dolphin. 



\noindent\textbf{Multi-Task Finetuning.} We additionally explore multitask learning \cite{caruana1997multitask,ruder2017overview} using our AraT5\textsubscript{v2} models. This strategy involves training the model on several tasks concurrently, allowing the model and its parameters to be shared across all tasks. The ultimate goal is to enhance performance on each individual task over time.




\subsection{Joint Pretraining and Finetuninig } 
In this scenario, we establish a uniform training objective for both pre-training and fine-tuning. The model is trained using a maximum likelihood objective, employing "teacher forcing" \cite{raffel2019exploring,williams1989learning} regardless of the specific task. To indicate the intended task for the model, we incorporate a task-specific (text) prefix to the original input sequence before presenting it to the model.









% \noindent\textbf{Dialectal Data (DA).} To create the Dialectal Data (DA) dataset, we utilize a corpus of $1.5$ billion Arabic tweets, which accounts for approximately $178$ GB of data. These tweets are randomly sampled from a larger in-house dataset comprising around $13$ billion Arabic tweets.

% \noindent\textbf{CA Data.} 
% We use the  Open Islamicate Texts Initiative (OpenITI) corpus  (v1.6)~\cite{nigst2020openiti}.\footnote{
% We exclude a random sample of $1$K books from  OpenITI for later use in evaluating~\ourmodel~ perplexity (see \cref{subsec:ppl}).} OpenITI  contains $11,195$ premodern Islamic books mainly collected from Shamela Liberay,\footnote{\href{https://shamela.ws}{https://shamela.ws}.} Al-Jami Al-Kabir collection (JK),\footnote{\href{http://kitab-project.org/docs/openITI}{http://kitab-project.org/docs/openITI}.} books digitized by Jordanian publisher Markaz Al-Turāth, and the Shia  Library.\footnote{\href{https://shiaonlinelibrary.com}{https://shiaonlinelibrary.com}.} \textbf{MSA Data.}  We use $\sim$$223$ GB of MSA text ($23.7$ billion tokens) from the following sources: AraNews\textsubscript{v2}~\cite{nagoudi2020machine},
% El-Khair~\cite{elkhair-2016}, Gigaword,\footnote{\href{https://catalog.ldc.upenn.edu/LDC2009T30}{https://catalog.ldc.upenn.edu/LDC2009T30}.} OSCAR~\cite{suarez2019asynchronous}, OSIAN~\cite{zeroual2019osian},  Wikipedia Arabic, and Hindawi Books.\footnote{\href{https://www.hindawi.org/books/}{https://www.hindawi.org/books}.} We also extract the Arabic part of the multilingual Colossal Clean Crawled Corpus (mC4)~\cite{xue2020mt5} and clean it (see ~\cref{subsec:pre_data} for cleaning procedure). We call the extracted portion AraC4 (more details are in Appendix~\ref{app:arac4}). \textbf{Dialectal Data (DA).} 
% We use a corpus of $1.5$ billion Arabic tweets ($178$GB) randomly sampled from a large in-house dataset of $\sim13$~billion Arabic tweets. 


